Nucleon-Gold Collisions at 200 AGeV Using Tagged d+Au Interactions in PHOBOS

Forward calorimetry in the PHOBOS detector has been used to study charged hadron production in d+Au, p+Au and n+Au collisions at sqrt(s_nn) = 200 GeV. The forward proton calorimeter detectors are described and a procedure for determining collision centrality with these detectors is detailed. The deposition of energy by deuteron spectator nucleons in the forward calorimeters is used to identify p+Au and n+Au collisions in the data. A weighted combination of the yield of p+Au and n+Au is constructed to build a reference for Au+Au collisions that better matches the isospin composition of the gold nucleus. The p_T and centrality dependence of the yield of this improved reference system is found to match that of d+Au. The shape of the charged particle transverse momentum distribution is observed to extrapolate smoothly from pbar+p to central d+Au as a function of the charged particle pseudorapidity density. The asymmetry of positively- and negatively-charged hadron production in p+Au is compared to that of n+Au. No significant asymmetry is observed at mid-rapidity. These studies augment recent results from experiments at the LHC and RHIC facilities to give a more complete description of particle production in p+A and d+A collisions, essential for the understanding the medium produced in high energy nucleus-nucleus collisions.

==> Makefile <==
# Makefile
# $Id: Makefile,v 1.3 2015/03/23 04:53:15 cjreed Exp $
#

FILENAME  = NucTagPaper

TEXDIR    = ./text
PICDIR    = ./img
TEXSRCS   = $(shell find $(TEXDIR) -maxdepth 1 -iname "*.tex") 
EPSPICS   = $(shell find $(PICDIR) -maxdepth 3 -iname "*.eps")
PICSRCS   = $(shell find $(PICDIR) -maxdepth 3 -iname "*.eps" \
              -or -iname "*.gif" -or -iname "*.jpeg" -or -iname "*.png")
PDFPICS   = $(patsubst %.eps,%.pdf,$(EPSPICS))

ARCH      = $(shell uname -s)
PDFTEX    = pdflatex
LATEX	  = latex
BIBTEX	  = ./sh/bibtex.sh
MKINDEX   = makeindex
PSVIEW    = gv
PDFVIEW   = acroread
DVIVIEW   = xdvi
DVIPS	  = dvips
PS2PDF    = ps2pdf
EPS2EPS   = eps2eps
EPSTOPDF  = epstopdf
THUMBPDF  = thumbpdf
EPSOPTION = 

ADDFILES  = $(FILENAME).tex $(FILENAME).bib Makefile ./sh/*.sh ./phobos_authors_dAu_revtex.tex ./data/Tables/*txt

#BACKFILES = $(PICSRCS) $(TEXSRCS) $(ADDFILES) 
BACKFILES = ./img/*pdf $(TEXSRCS) $(ADDFILES) 

all:		 	$(FILENAME).pdf

$(FILENAME):		$(FILENAME).tex $(TEXSRCS) $(EPSPICS) $(ADDFILES)
	$(LATEX) 	$(FILENAME)

$(FILENAME).pdf:	$(FILENAME).tex $(TEXSRCS) $(PDFPICS) $(ADDFILES)
	$(PDFTEX) 	$(FILENAME)
	$(BIBTEX) 	$(FILENAME)
#	$(MKINDEX)	$(FILENAME)
	$(PDFTEX) 	$(FILENAME)
#	$(THUMBPDF)     $(FILENAME)
	$(PDFTEX) 	$(FILENAME)

$(FILENAME).dvi:	$(FILENAME).tex $(TEXSRCS) $(EPSPICS) $(ADDFILES)
	$(LATEX) 	$(FILENAME)
	$(BIBTEX) 	$(FILENAME)
#	$(MKINDEX) 	$(FILENAME)
	$(LATEX) 	$(FILENAME)
	$(LATEX) 	$(FILENAME)

$(FILENAME).ps:		$(FILENAME).dvi
	$(DVIPS) 	$(FILENAME).dvi -o $(FILENAME).ps

ps: 	$(FILENAME).ps

gzip:	$(FILENAME).ps
	gzip $(FILENAME).ps

pdf: 	$(FILENAME).pdf

rpdf: 	
	$(PDFTEX) 	$(FILENAME)

ps2pdf:	$(FILENAME).dvi
	$(DVIPS) -Ppdf $(FILENAME).dvi -o $(FILENAME).ps
	$(PS2PDF) $(FILENAME).ps

vdvi:	$(FILENAME).dvi
	$(DVIVIEW) $(FILENAME).dvi

vps:	$(FILENAME).ps
	$(PSVIEW) $(FILENAME).ps

vpdf:	$(FILENAME).pdf
	$(PDFVIEW) $(FILENAME).pdf

print:  $(FILENAME).ps
	lpr $(FILENAME).ps

$(FILENAME).tar.gz:	backup

backup:
	tar -cvzf $(FILENAME).tar.gz $(BACKFILES)

sbackup:
	tar -cvzf $(FILENAME).tar.gz $(BACKFILES)
	scp -p $(FILENAME).tar.gz rftpexp.rhic.bnl.gov:~/backup

dbackup: 
	tar -cvzf ./backup/$(FILENAME)-backup`./sh/dbackup.sh $(FILENAME) backup 5`.tar.gz $(BACKFILES)

#sdbackup: dbackup
#	scp -p ./backup/$(FILENAME)-backup`cat ./backup/.arbeit-count`.tar.gz pcikf27.ikf.physik.uni-frankfurt.de:~/backup

clean:
	rm -f $(FILENAME).ps $(FILENAME).pdf $(FILENAME).tar.gz \
	rm -f $(FILENAME).dvi \
	$(FILENAME).toc $(FILENAME).aux $(FILENAME).out \
	$(FILENAME).bbl $(FILENAME).blg $(FILENAME).log \
	$(FILENAME).lof $(FILENAME).lot $(FILENAME).idx \
	$(FILENAME).ind $(FILENAME).ilg $(FILENAME).glo \
	$(FILENAME).blg $(FILENAME).brf \
        texput.log core .tmp.eps 

cleangen:
	rm -f $(FILENAME).toc \
        $(FILENAME).bbl $(FILENAME).blg $(FILENAME).lof \
        $(FILENAME).lot $(FILENAME).idx $(FILENAME).ind \
        $(FILENAME).ilg $(FILENAME).glo $(FILENAME).blg \
        $(FILENAME).brf

realclean: clean
	rm -f $(FILENAME).ps $(FILENAME).pdf $(FILENAME).tar.gz \
	$(PDFPICS) fmffig*
	find . -type f -name "*~" -exec rm -f "{}" \;
	find . -type d -exec chmod 755 "{}" \;
	find . -type f -exec chmod 644 "{}" \;
	find . -name "*.sh" -type f -exec chmod 755 "{}" \;

.phony: clean print backup sbackup dbackup sdbackup rpdf

$(PDFPICS): %.pdf: %.eps
ifeq ($(ARCH),Darwin)
	perl -i -pe 's/\015/\012/g' $<
endif
	$(EPSTOPDF) $(EPSOPTION) $< --outfile=$@
#	$(EPS2EPS) $< .tmp.eps && $(EPSTOPDF) $(EPSOPTION) .tmp.eps --outfile=$@ && rm -f .tmp.eps

